Differential Privacy for Text Analytics via Natural Text Sanitization

Texts convey sophisticated knowledge. However, texts also convey sensitive information. Despite the success of general-purpose language models and domain-specific mechanisms with differential privacy (DP), existing text sanitization mechanisms still provide low utility, as cursed by the high-dimensional text representation. The companion issue of utilizing sanitized texts for downstream analytics is also under-explored. This paper takes a direct approach to text sanitization. Our insight is to consider both sensitivity and similarity via our new local DP notion. The sanitized texts also contribute to our sanitization-aware pretraining and fine-tuning, enabling privacy-preserving natural language processing over the BERT language model with promising utility. Surprisingly, the high utility does not boost up the success rate of inference attacks.

==> Tables/old_Table1.tex <==
%!TEX root = main.tex

\begin{table*}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|l|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{ \textbf{\begin{tabular}[c]{@{}c@{}}Eval\\ Settings\end{tabular}}}} & \multirow{2}{*}{\textbf{Mechanisms}} & \multicolumn{3}{c|}{\textbf{SST-2}} & \multicolumn{3}{c|}{\textbf{CliniSTS}} & \multicolumn{3}{c}{\textbf{QNLI}} \\ \cline{3-11} 
 & &  $\epsilon=1$ & $\epsilon=2$ & $\epsilon=3$ & $\epsilon=1$ & $\epsilon=2$ & $\epsilon=3$ & $\epsilon=1$ & $\epsilon=2$ & $\epsilon=3$ \\ \hline\hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sanitized \\ Test\end{tabular}}} & Random &
$0.4986$ &	$0.4986$	&$0.4986$	&	$0.0196$	&	$0.0196$	&	$0.0196$ & $0.5152$  & $0.5152$ &$0.5152$
\\ \cline{2-11} 
 & CMP &$0.5099$  &$0.5143$  &$0.5345$  &$0.0201$  &$0.0361$  &$0.0452$ &$0.5162$  & $0.5256$ &$0.5333$ \\ \cline{2-11} 
 & \baseDP &
$0.5101$ &	$0.5838$	&	$0.8374$	&	$0.0351$	&	$0.5392$	&	$0.8159$ & $0.5372$  & $0.5598$  &$0.8116$
\\ \cline{2-11} 
 & \textbf{\baseDPp} &$0.7796$ &$0.7943$  &$0.8516$
&$0.4965$ &$0.7082$  &$0.8162$   &$0.7699$  &$0.7760$ &$0.8131$\\ \hline \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Real \\ Test\end{tabular}}} & Random &  
$0.5115$    &   $0.5115$    &   $0.5115$    &   $0.0230$    &   $0.0230$    &   $0.0230$ & $0.5059$  &$0.5059$  &$0.5059$
\\ \cline{2-11} 
& CMP &$0.5226$ &$0.5376$  &$0.5469$  &$0.1024$ &$0.1456$  &$0.1638$  &$0.5234$  &$0.5336$ &$0.5454$
\\ \cline{2-11} 
 & \baseDP &
$0.5560$ &	$0.7973$	&	$0.9169$    &   $0.1401$    &   $0.6826$    & $0.8522$ & $0.5315$  & $0.5569$  & $0.8679$
\\ \cline{2-11} 
 & \textbf{\baseDPp} &$0.8879$ &$0.8976$  &$0.9170$  &$0.6621$ &$0.7783$  &$0.8566$ &$0.8576$  &$0.8617$ &$0.8762$ \\ \hline \hline
\textbf{Optimal} &  & \multicolumn{3}{c|}{$0.9251$} & \multicolumn{3}{c|}{$0.8527$} & \multicolumn{3}{c}{$0.9090$} \\ \hline
\end{tabular}
}
\caption{Comparison of utilities of different DP mechanisms under similar privacy levels: Our context-aware sanitized mechanism \baseDP achieve the best performance in all the evaluation settings of the three tasks.
}
\label{tbl:comparison}
\vspace{-10pt}
\end{table*}

==> Tables/old_Table2.tex <==
%!TEX root = main.tex

\begin{table}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{$\epsilon$}} & \multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Privacy}} \\ \cline{3-6} 
 &  & Original & +Pretrain & Original & +Pretrain \\ \hline
\multirow{3}{*}{\textbf{SST-2}} & 12 &0.6084  &\textbf{0.6208} &0.9219  &{0.9308}  \\ \cline{2-6} 
 & 14 & 0.7548  &\textbf{0.7731}  & 0.8205  & {0.8306} \\ \cline{2-6} 
 & 16 & 0.8698   &\textbf{0.8830}   & {0.6243}  & 0.6197 \\ \hline\hline
\multirow{3}{*}{\textbf{QNLI}} & 12 & 0.5822   & \textbf{0.6037}  &0.9508  &0.9584  \\ \cline{2-6} 
 & 14 &0.7143  &\textbf{0.7309} &0.8430  &0.8383  \\ \cline{2-6}
 & 16 &0.8265 & \textbf{0.8369} &0.6438  &0.6399  \\ \hline
\end{tabular}
}
\caption{Results of Sanitization-based pretraining}
\vspace{-10pt}
\label{tbl:comparisonModel}
\end{table}
